False Discovery Control in Multiple Testing: A Brief Overview of Theories and Methodologies

As the volume and complexity of data continue to expand across various scientific disciplines, the need for robust methods to account for the multiplicity of comparisons has grown widespread. A popular measure of type 1 error rate in multiple testing literature is the false discovery rate (FDR). The FDR provides a powerful and practical approach to large-scale multiple testing and has been successfully used in a wide range of applications. The concept of FDR has gained wide acceptance in the statistical community and various methods has been proposed to control the FDR. In this work, we review the latest developments in FDR control methodologies. We also develop a conceptual framework to better describe this vast literature; understand its intuition and key ideas; and provide guidance for the researcher interested in both the application and development of the methodology.

==> main/MT_sideinfo.tex <==
\section{Multiple Hypotheses Testing with Side Information}	\label{sec:sideinfo}
Conventional multiple testing procedures implicitly assume that data are collected from repeated or identical experimental conditions, implying that hypotheses are exchangeable. However, in many applications, data are known to be collected from heterogeneous sources. Moreover, relevant domain knowledge, such as carefully constructed auxiliary sequences from the same dataset \citep{liu2014incorporation,tony2019covariate} and external covariates or prior data from secondary data sources \citep{fortney2015genome,scott2015false,ignatiadis2016data,zhang2022covariate}, is often available alongside the primary dataset in many studies. Furthermore, side information can be categorized as follows: (\romannumeral1) continuous variables, including the minor allele frequency, the prevalence of bacterial species in genetics, and sample variance of experiments; (\romannumeral2) discrete variables, including location in 1D, 2D, or 3D coordinate systems from satellite monitoring and neuroimaging, and order of gene expression data when dealing with RNA-Seq; (\romannumeral3) categorical variables, including the affiliations or sub-groups. See Figure \ref{fig:side_info} for an illustration. For instance, consider testing for the association of 400,000 single-nucleotide polymorphisms (SNPs) with each of 40 related diseases. If gene-regulatory relationships are known, then we could expect SNPs near genes to be associated with related diseases. 

Following this, extensive research efforts have been devoted to grouped hypotheses testing \citep{cai2009simultaneous,hu2010false}, ordered hypotheses testing \citep{lei2016power,li2017accumulation}, and covariate-adjusted hypotheses testing \citep{ignatiadis2016data,lei2018adapt,zhang2022covariate,leung2022zap} to fully exploit the power of statistical inference when external or structural information is provided. Since the grouped and order hypotheses testing can be viewed as special cases of the covariate-adjusted testing, the problem with side information can generally be framed as the covariate-regulated models. For each hypothesis, the practitioner obseves a summary statistics $X_i\in\RR$ alongside a covariate $s_i\in\cS$ with $\cS\subseteq\RR^d$. Following the literature, we consider a two-component mixture model:
\begin{equation}\label{eq:bayes_model_side}
\theta_i\overset{\rm iid}{\sim}{\rm Bernoulli}(\pi_{s_i})\quad X_i|s_i\overset{\rm iid}{\sim} (1-\theta_i)f_{0}+\theta_if_{1,s_i},\quad\forall i\in\cM,
\end{equation}
where the null distribution $f_{0}$ under $H_{0,i}$ is specified and the non-null distribution $f_{1,s_i}$  under $H_{1,i}$ is unknown. Compared to the conventional two-component mixture model in \eqref{eq:bayes_model}, the varying null probability $\pi_{s_i}$ reflects the relative importance of each hypothesis given the covariate information $s_i$ and the varying alternative density $f_{1,s_i}$ emphasizes the heterogeneity among the signals. In this section, we introduce two main approaches towards covariate-adjusted testings: weighted BH (see \S\ref{sec:WBH}) and generalized BC procedure (see \S\ref{sec:GBC}). These approaches are extensions of the standard BH and BC procedures discussed in \S\ref{sec:BH} and \S\ref{sec:BC}, respectively.
\begin{figure}[t]
  \centering
  \begin{minipage}[b]{0.66\textwidth}
    \centering
    \includegraphics[width=1\textwidth]{fig/Fig.2.1.pdf}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.33\textwidth}
    \centering
    \includegraphics[width=1\textwidth]{fig/Fig.2.2.pdf}
  \end{minipage}
  \caption{Illustrations of informative side information in multiple testing: ordered hypotheses (left) with shaded area as potentially significant features ($\pi_i>0$), and two-dimensional clustering pattern (right) on a 100$\times$100 lattice with blue dots as the ground-truth features with $\pi=0.8$.}
  \label{fig:side_info}
\end{figure}
\subsection{Weighted BH (WBH) Procedure}\label{sec:WBH}
Weighting is a widely used strategy for incorporating side information into FDR analyses \citep{benjamini1997multiple,genovese2006false,basu2018weighted}. Following the literature, let $(\omega_i)_{i\in\cM}$ be a set of weights, where the collected p-values $(P_i)_{\in\cM}$ is independent of weights $(\omega_i)_{i\in\cM}$ conditioned on the set of null hypotheses $\cH_0$. The WBH procedure can summarized below:
\begin{equation}
	\textbf{WBH:}\quad T_i=P_i/w_i,\quad \widehat{\rm FDP}(t)=\frac{mt}{\sum_{i=1}^m\ind(P_i/w_i\leq t)},
	\label{eq:WBH}
	\end{equation}
where the WBH procedure is equivalently using $P_i/\omega_i$'s as the input of standard BH procedure. The following theorem posits that WBH procedure ensures FDR control under certain regulations.
 \begin{theorem}\label{thm:WBH}
 Suppose that $(P_i)_{\in\cM}$ is independent of $(\omega_i)_{i\in\cM}$ conditioned on  $\cH_0$ with $\sum_{i\in\cH_0}\omega_i\leq m$. The WBH procedure controls FDR at level $\alpha$ in finite sample.
 \end{theorem}
 
 \begin{proof}[Sketch]%[Sketch proof of Theorem \ref{thm:WBH}] 
 The proof is akin to that of Theorem \ref{thm:BH}. Let $\alpha_j=\alpha j /m$ and $\cR_{t_\alpha,i\rightarrow 0}$ be the rejection set by apply BH procedures on $(P_i)_{i\in\cM}$ with $P_i$ substituted by 0
\begin{align} 
\mathbb{E}\left[\dfrac{|\cR_{t_\alpha}\cap\cH_0|}{|\cR_{t_\alpha}|\vee 1}\right]&=
\sum_{i\in \cH_0}  \sum_{j=1}^m \frac{1}{j}\cdot \EE\left[\ind(|\cR_{t_\alpha}| = j)\cdot\ind\left(P_i\leq\omega_i\cdot\alpha_j\right)\right]\notag\\
&=\sum_{i\in \cH_0}\sum_{j=1}^m\PP(P_i\leq\omega_i\cdot\alpha_j)\cdot\PP(|\cR_{t_\alpha,i\rightarrow 0}| = j)\notag\\
&=\sum_{i\in \cH_0} \sum_{j=1}^m\frac{\omega_i}{j}\cdot\frac{\alpha j}{m}\cdot\PP(|\cR_{t_\alpha,i\rightarrow 0}| = j)=\frac{\alpha}{m}\sum_{i\in\cH_0}\omega_i\leq\alpha,
\end{align}
where the third equation results from conditional independence and the inequality follow $\sum_{i\in\cH_0}\omega_i\leq m$. Then, we complete the proof of Theorem \ref{thm:WBH}.
\end{proof}	
The original condition in \cite{genovese2006false} requires $\sum_{i\in\cM}\omega_i\leq m$, which is slightly stronger than the one we used. Here, we provide an intuition behind the weight condition. For exchangeable hypotheses, as demonstrated in \S\ref{sec:adaBH}, we can use BH procedure at level $m\alpha/|\cH_0|$ as a remedy for the over-conservativeness, which is equivalently using $P_i/\omega_i$ with weight $\omega_i=m/|\cH_0|$. To accommodate the side information into the testing procedure, \cite{li2017accumulation} proposed to use $\omega_i=\frac{1}{1-\pi(s_i)}$, which is a natural extension to $\omega_i=m/|\cH_0|$ under the model in \eqref{eq:bayes_model_side}; and \cite{cai2022laws} suggested using $\omega_i=\frac{\pi(s_i)}{1-\pi(s_i)}$ to separate the clustered nonnull p-values more effectively, motivated by the optimality theory in \cite[\S 4.1,][]{tony2019covariate}, which we will discuss in detail later. We remark that both weights are valid under regulations, and the main challenge lies in estimating function $\pi_s$ from data. For instance, \cite{cai2022laws} proposed a model-free estimation via screening:
\begin{equation}
	\hat{\pi}_\lambda(s)=1-\frac{\sum_{i=1}^m\cK_h(s,s_i)\ind(P_i\geq\lambda)}{(1-\lambda)\cdot\sum_{i=1}^m\cK_h(s,s_i)},\quad\forall\lambda\in(0,1),
	\label{eq:law_nonnull}
\end{equation}
where $\cK_h:\RR^d\times\RR^d\mapsto\RR$ is a positive, bounded, and symmetric kernel function with bandwidth $h$ chosen by cross-validation. The estimation in \eqref{eq:law_nonnull} can be viewed as a kernelized Storey's $\hat{\pi}_0$ in \eqref{eq:storeypi}, screening over the collected side information $\{s_i\}_{i\in\cM}$. We remark that WBH procedure with weights constructed upon covariate-adjusted non-null proportions shows significant power improvement with mild conditions. However, it still has limitations: (\romannumeral1) it neglects the varying alternative density $f_{1,s_i}$ that emphasizes the heterogeneity among the signals; (\romannumeral2) given the low convergence rate of kernel methods, the estimation of non-null is not that accurate in practical settings, leading to power loss. Fortunately, statisticians have developed the optimal theories and a series of powerful ``distribution-free" tools to address these issues, which we will discuss in detail in the next section.
	
\subsection{Generalized BC (GBC) Procedure}\label{sec:GBC}
Following the covariate-adjusted two-component mixture model in \eqref{eq:bayes_model_side}, \cite{tony2019covariate} showed that the optimal procedure for the covariate-adjusted testings is the ranking and thresholding procedure upon the conditional local false discovery rate (Clfdr), defined as
\begin{equation}
	\label{eq:clfdr}
		\text{Clfdr}_{s_i}(X_i)=\mathbb{P}(\theta_i=0|X_i,s_i)=\frac{(1-\pi_{s_i})f_{0}(X_i)}{(1-\pi_{s_i})f_{0}(X_i)+\pi_{s_i} f_{1,s_i}(X_i)}.
\end{equation}
Some astute readers may observe that practitioners could apply SC procedure over estimated Clfdr's to control FDR with covariate adjustment. However, as discussed in \S \ref{sec:WBH}, $\pi_s$ is hard to estimate, especially in the presence of multi-dimensional side information, since the convergence rate increases exponentially with dimension $d(\cS)$, let alone estimating the entire Clfdr. To address these issues, \cite{lei2018adapt} first proposed a two-fold solution. First, they suggested using a model-based method to estimate $\widehat{\text{Clfdr}}_s$, leading to a faster convergence rate. Second, they proposed controlling FDR using a ``distribution-free" filter---generalized BC procedure. This approach provides theoretical guarantees regardless of the accuracy of $\widehat{\text{Clfdr}}_s$ estimator. Here, we adopt the GBC procedure proposed by \cite{leung2022zap}, which is a natural generalization of the method used in \cite{lei2018adapt,zhang2022covariate}, sharing a similar high-level idea. Let $\cA:\RR\times\cS\mapsto\RR$ be an assessor function that approximates Clfdr, i.e., $\widehat{\text{Clfdr}}_s(X)=\cA(X,s)$, and $c_s(t)=\PP(\cA(X,s)\leq t|H_0,s)$ be the conditional CDF under the null. Suppose that $c_s$ is continuous and strictly increasing. Following this, the GBC procedure can be summarized as
\begin{equation}
\textbf{GBC:}\quad T_i=\cA(X_i,s_i),\quad \widehat{\rm FDP}(t)=\frac{1+\sum_{i=1}^m\ind(c_{s_i}(\cA(X_i,s_i))\geq1-c_{s_i}(t))}{\sum_{i=1}^m\ind(\cA(X_i,s_i)\leq t)},
\label{eq:GBC}
\end{equation}
and the candidate rejection is chosen as $\cT=(0,t_{\rm max}]$ with $t_{\max}=\max\{t:c_{s_i}(t)\leq 0.5\text{~for all~}i\}$. The intuition behind the GBC estimator in \eqref{eq:GBC} is straightforward. It constructs covariated-adjusted p-values $c_{s_i}(\cA(X_i,s_i))$ using the known $f_0$. Specifically, the FDR control is realized via
	\begin{align*}
		\text{FDP}(\mathcal{R}_{t_\alpha})&<\dfrac{1+\sum_{i\in\cH_0}\ind(\cA(X_i,s_i)\leq t)}{\sum_{i=1}^m\ind(\cA(X_i,s_i)\leq t)\vee1}\\
		&=\dfrac{1+\sum_{i\in\cH_0}\ind(c_{s_i}(\cA(X_i,s_i))\leq c_{s_i}(t))}{\sum_{i=1}^m\ind(\cA(X_i,s_i)\leq t)\vee1}\\ 
		&\approx\dfrac{1+\sum_{i\in\cH_0}\ind(c_{s_i}(\cA(X_i,s_i))\geq 1-c_{s_i}(t))}{\sum_{i=1}^m\ind(\cA(X_i,s_i)\leq t)\vee1},
	\end{align*}
	where the $``\approx"$ follows from the fact that $c_{s_i}(\cA(X_i,s_i))$ is a uniformly distributed random variable over $[0,1]$ under $H_{0,i}$. The following theorem shows that given pre-determined assessor function $\cA$, the GBC procedure ensures a finite-sample FDR guarantee at designated level $\alpha\in(0,1)$.
	
\begin{figure}[!t]
\centering
\includegraphics[width=0.7\linewidth]{fig/fig4.1.pdf}
\includegraphics[width=0.7\linewidth]{fig/fig4.2.pdf}
\caption{Numerical results of the covariate-adjusted procedures, with \texttt{AdaPT} proposed by \cite{lei2018adapt} used as an example of GBC procedures: continous cases (left) follows normal mixture model $Z_i\sim(1-\pi_{s_i})\cdot\cN(0,1)+\pi_{s_i}\cdot\cN(\mu_{s_i},1)$ with $s_i\sim{\rm Unif}[0,1]$, $\pi_{s_i}=s_i^2/2$, and $\mu_{s_i}=s_i\mu$; discrete cases (right) follows $X_i\sim(1-\pi_{s_i})\cdot\cN(0,1)+\pi_{s_i}\cdot\cN(\mu,1)$ with $s_i=i$ and $\pi_{s_i}$ is set as the ordering case in Figure \ref{fig:comparison_stats}. Here, $\mu$ varies from $2$ to $4$, and $P_i=2\Phi(-|Z_i|)$ is normalized in correspondence.}
\label{fig:comparison_side}
\end{figure}  
\begin{theorem}\label{thm:GBC}
Let $\mathcal{A}:\mathbb{R}\times\cS\rightarrow\mathbb{R}$ be a pre-determined assessor function and $c_s:\RR\mapsto\RR$ be the null CDF in correspondence. The GBC procedure controls FDR at $\alpha$ in finite sample.
\end{theorem}
\begin{proof}%[Proof of Theorem \ref{thm:GBC}]
	The proof is akin to that of Theorem \ref{thm:BC}. Please refer to \S\ref{ap:GBC} for details. 
\end{proof}
We remark that the assessor-based GBC procedure is favorable as the FDR guarantee does not depend on the quality of approximation for Clfdr, which is desirable as Clfdr is extremely hard to estimate in practice and only affects the power of the testing procedure. Besides, compared with directly apply BH or BC procedure on covariate-adjusted p-values $c_{s_i}(\cA(X_i,s_i))$'s, the GBC procedure outperforms by ranking with $\cA(X_i,s_i)$'s, i.e., the assessor of ${\rm Clfdr}_{s_i}(X_i)$'s, aligning with the optimal theory that suggests a Clfdr-based procedure. For illustration, we briefly introduce the three-component beta-mixture model in \cite{leung2022zap}, formulated as
	$$
	\Phi(X_i)|s_i\sim\{1-\pi_l(s_i)-\pi_r(s_i)\}h_0(\cdot)+\pi_l(s_i)h_l(\cdot)+\pi_r(s_i)h_r(\cdot), \quad\forall i\in\cM,
	$$
	where $\Phi:\RR\mapsto[0,1]$ is a regulation function, the conditional non-null proportions $\pi_l(\cdot)$, $\pi_r(\cdot)$ are characterized by softmax distributions and the density functions $h_l(\cdot)$, $h_r(\cdot)$ follow beta distributions.Specifically, let $\tilde{s}_i=(1,s_i)$ and the non-null proportion is then modeled as
	$$
	\pi_{l}(s_i)=\frac{\exp(\theta_l^\top\tilde{s}_i)}{1+\exp(\theta_l^\top\tilde{s}_i)+\exp(\theta_r^\top\tilde{s}_i)},\quad \pi_{r}(s_i)=\frac{\exp(\theta_l^\top\tilde{s}_i)}{1+\exp(\theta_r^\top\tilde{s}_i)+\exp(\theta_r^\top\tilde{s}_i)},
	$$
	and the conditional density function follows
	$$
	h_l(u)=B(k_l(s_i),\gamma_l)^{-1} u^{k_l(s_i)-1}(1-u)^{\gamma_l},\quad h_l=r(u)=B(k_r(s_i),\gamma_r)^{-1} u^{k_r(s_i)-1}(1-u)^{\gamma_r},
	$$
	where $k_l(s)=\{1+\exp(-\beta_l^\top\tilde{s})\}^{-1}$ and $k_r(s)=\{1+\exp(-\beta_r^\top\tilde{s})\}^{-1}$. Following this, the practitioners can estimate the parameters using EM algorithms. The beta mixture model has long been identified as a flexible modeling tool for variables taking values in the unit interval \citep{parker1988identifying,ferrari2004beta,markitsis2010censored}, and similar models are adopted in \cite{lei2018adapt,zhang2022covariate,leung2022zap} for covariate-adjusted testings. However, such methodology still has limitations: (\romannumeral1) as noted earlier, the power of testing procedure relies heavily on the choice of assessor model, which is manually decided; (\romannumeral2) while GBC ensures a finite-sample FDR control with a pre-determined assessor, in practice such an assessor is estimated from data, resulting in degradation to asymptotic control. This is because estimated $\hat{\mathcal{A}}$ is not independent of ${(X_i,s_i)}_{i\in\mathcal{M}}$, and Theorem \ref{thm:GBC} no longer holds. To avoid dependence, the data-driven conclusion is achieved by showing that: firstly, by using an oracle assessor, i.e., $\mathcal{A}^*$ that maximizes the risk of the EM algorithms, finite-sample is ensured following Theorem \ref{thm:GBC}. Secondly, show that the data-driven $\hat{\mathcal{A}}$ is a consistent estimation of oracle $\mathcal{A}^*$ based on the property of EM estimators \citep{mclachlan2007algorithm}. See \cite{zhang2022covariate,leung2022zap} for detailed proof of data-driven procedures. Moreover, \cite{lei2018adapt,leung2022zap} developed an iterative approach with slight modifications to achieve finite-sample control. Very recently, \cite{gang2023unified,li2023values} proposed generalized BH (GBH) procedures, which share a similar idea introduced in this section. Please see these papers for further discussions.
	
	












